Super-resolved Lasso

Super-resolution of pointwise sources is of utmost importance in various areas of imaging sciences. Specific instances of this problem arise in single molecule fluorescence, spike sorting in neuroscience, astrophysical imaging, radar imaging, and nuclear resonance imaging. In all these applications, the Lasso method (also known as Basis Pursuit or \( \ell^1 \)-regularization) is the de facto baseline method for recovering sparse vectors from low-resolution measurements. This approach requires discretization of the domain, which leads to quantization artifacts and consequently, an overestimation of the number of sources. While grid-less methods, such as Prony-type methods or non-convex optimization over the source position, can mitigate this, the Lasso remains a strong baseline due to its versatility and simplicity. In this work, we introduce a simple extension of the Lasso, termed ``super-resolved Lasso" (SR-Lasso). Inspired by the Continuous Basis Pursuit (C-BP) method, our approach introduces an extra parameter to account for the shift of the sources between grid locations. Our method is more comprehensive than C-BP, accommodating both arbitrary real-valued or complex-valued sources. Furthermore, it can be solved similarly to the Lasso as it boils down to solving a group-Lasso problem. A notable advantage of SR-Lasso is its theoretical properties, akin to grid-less methods. Given a separation condition on the sources and a restriction on the shift magnitude outside the grid, SR-Lasso precisely estimates the correct number of sources.

==> sections/applications.tex <==
% !TEX root = ../Paper.tex
\section{Applications}
\label{sec:applis}
\setlength{\tabcolsep}{5pt}


\paragraph{Evaluation metric}
Maximum mean discrepancy (MMD) norms \cite{} over complex measures (which is a special case of vector valued measures) are defined, for some positive kernel $k(x,y)$ as 
$$
    \|\mu\|_k^2 := \int k(x,y) \text{d}\mu(x) \bar \mu(y).
$$
We consider the Laplace kernel $k(x,y) = \exp(-\norm{x-y})$ and let
$$
D(\mu,\nu) = \| \mu -  \nu\|_k^2.
$$
For all measures $\mu,\nu$, we have $D(\mu,\nu)\geq 0$ and $D(\mu,\nu) = 0$ if $\mu=\nu$ \todo{is this if and only if?}
Note that our loss term can be seen as minimising MMD with kernel $k(x,y) = \phi(x)^\top \phi(y)$. Since the Laplace kernel has slow Fourier decay, in using the Laplace kernel instead for evaluation, this intuitively  measures the match on ``higher order moments". %Note that $$D(a_1\delta_{x_1}, a_2 \delta_{x_2}) = a_1^2 + a_2^2 - 2a_1 a_2 \exp(-|x_1-x_2|).$$


%We consider the energy distance kernel $k(x,y) = -\norm{x-y}$ and this is a distance \todo{is this true} over measures that have the same total mass, that is $\int d\mu = \int d\nu$. In this section, to evaluate the performance of the different algorithms, we consider the following metric
%$$
%D(\mu,\nu) = \| \bar \mu - \bar \nu\|_j^2 + \gamma \abs{\norm{\mu}_1  - \norm{\nu}_1},
%$$
%for some weight $\gamma>0$ and  where $\bar \mu = \mu - c \chi_{\Supp(\mu)}$ and $\bar \nu = \nu +  c \chi_{\Supp(\nu)}$ have equal mass. That is,
%$$
%c = (\abs{\Supp(\nu)} +  \abs{\Supp(\mu)} )^{-1}\pa{\int d\mu -  \int d\nu}.
%$$ 


\subsection{Fourier in 1D}
Let $f_c = 3$ and $$\Phi \mu = \pa{\int \exp(-2\pi i k x) \mathrm{d}\mu(x)}_{\abs{k}\leq f_c}.$$
In this section, to illustrate the influence of $\tau$, we carry out the following procedure:
Assume that the reconstruction grid is a uniform grid spaced $1/N$ apart.
The data $\Phi \mu_0$ is generated from the sparse measure
$$
\mu_0 = 2\delta_{x_1+ h/N} + \delta_{x_2-h_1/N },
$$
where $ h$  is the fraction that we move inside the grid. The observed signal is noise-corrupted with
\begin{equation}\label{eq:noisy_y}
y =  y_0+ \Nn(0, \rho^2 \Id_{MT}), \qwhereq y_0 \eqdef \Phi \mu_0 \qandq \rho \eqdef 0.1 \frac{\norm{y_0}}{\sqrt{MT}}.
\end{equation}
In Table \ref{tab:fourier}, we show the influence of changing $h$ on $\tau$ and the reconstruction. Given $h$, we carry out the following computations:
\begin{enumerate}
\item Find the optimal $\lambda_*$ parameter for Lasso. We do this by searching over a grid of size 20 on $[0,\lambda_{\max}]$ where we let $\lambda_{\max} = \norm{X^\top y_0}_\infty$. For each $\lambda$ value on this grid, we compute
$$
E_{L}(\lambda)\eqdef \frac{1}{10} \sum_{i=1}^{10} D(\mu_0, \mu_{\mathrm{Lasso}}(\lambda,y_i) )
$$
for 20 instances of $y_i$ distribution as in \eqref{eq:noisy_y} and choose  $\lambda_*$ as the parameter with the smallest $E(\lambda)$ value.
\item For this given $\lambda_*$, searching over 20 uniformly spaced points for $\tau$ in $[0,1]$, we compute 
$$
E_{SR}(\lambda_*,\tau)\eqdef \frac{1}{10} \sum_{i=1}^{10} D(\mu_0, \mu_{\mathrm{SR-Lasso}}(\lambda_*,\tau,y_i) )
$$
where the sum is over  10 instances of $y_i$ distribution as in \eqref{eq:noisy_y}. The   $\tau$   with the smallest $E_{SR}(\lambda_*,\tau)$ value is recorded in Table \ref{tab:fourier}. Graphs of $\tau \mapsto E_{SR}(\lambda_*,\tau)$ with error bars are shown in Figure \ref{fig:fourier10}, \ref{fig:fourier20} and \ref{fig:fourier30} in the cases $N=10,20,30$. Observe that when $h=0$ (the true Diracs are on the grid), the optimal $\tau$ value is 0, whereas, as $h$ increases, the optimal $\tau$ values increase as more movement inside the grid is desirable. 
\end{enumerate}

\begin{table}
\begin{center}
\begin{tabular}{c|c|c|c|c|c|}
$N$&$h$&$\tau$&$\lambda$&$\mathrm{Err}_{L}$&$\mathrm{Err}_{SR}$\\\hline
$10$&$0.00$&$0.00$&$0.131$&$0.068$&$0.068$\\
$10$&$0.10$&$0.89$&$0.129$&$0.248$&$0.139$\\
$10$&$0.20$&$1.00$&$0.183$&$0.392$&$0.161$\\
$10$&$0.30$&$1.00$&$0.176$&$0.494$&$0.206$\\
$10$&$0.40$&$1.00$&$0.244$&$0.558$&$0.275$\\\hline
$20$&$0.00$&$0.00$&$0.131$&$0.073$&$0.073$\\
$20$&$0.10$&$0.56$&$0.130$&$0.159$&$0.128$\\
$20$&$0.20$&$0.78$&$0.129$&$0.229$&$0.149$\\
$20$&$0.30$&$0.89$&$0.186$&$0.277$&$0.166$\\
$20$&$0.40$&$1.00$&$0.183$&$0.306$&$0.182$\\\hline
$30$&$0.00$&$0.00$&$0.191$&$0.083$&$0.083$\\
$30$&$0.10$&$0.56$&$0.190$&$0.135$&$0.118$\\
$30$&$0.20$&$0.78$&$0.189$&$0.179$&$0.134$\\
$30$&$0.30$&$0.89$&$0.188$&$0.212$&$0.153$\\
$30$&$0.40$&$0.89$&$0.186$&$0.230$&$0.169$
\end{tabular}
\end{center}

\caption{Reconstruction from Fourier measurements with $f_c = 3$.\label{tab:fourier}}
\end{table}


\setlength{\tabcolsep}{0pt}

\begin{figure}
\begin{tabular}{cccccc}
\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_10_0/tau_SRLasso}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_10_10/tau_SRLasso}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_10_20/tau_SRLasso}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_10_30/tau_SRLasso}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_10_40/tau_SRLasso}\\
\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_10_0/comparison}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_10_10/comparison}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_10_20/comparison}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_10_30/comparison}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_10_40/comparison}
\end{tabular}
\caption{$N=10$ and $f_c = 3$. Top row shows the error as we change $\tau$. The results are averaged over $20$ random noisy instances.Bottom row shows the reconstruction for one particular noisy instance.\label{fig:fourier10}}
\end{figure}


\begin{figure}
\begin{tabular}{cccccc}
\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_20_0/tau_SRLasso}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_20_10/tau_SRLasso}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_20_20/tau_SRLasso}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_20_30/tau_SRLasso}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_20_40/tau_SRLasso}\\
\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_20_0/comparison}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_20_10/comparison}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_20_20/comparison}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_20_30/comparison}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_20_40/comparison}
\end{tabular}
\caption{$N=20$ and $f_c = 3$. Top row shows the error as we change $\tau$. The results are averaged over $20$ random noisy instances.Bottom row shows the reconstruction for one particular noisy instance. \label{fig:fourier20}}
\end{figure}

\begin{figure}
\begin{tabular}{cccccc}
\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_30_0/tau_SRLasso}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_30_10/tau_SRLasso}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_30_20/tau_SRLasso}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_30_30/tau_SRLasso}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_30_40/tau_SRLasso}\\
\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_30_0/comparison}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_30_10/comparison}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_30_20/comparison}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_30_30/comparison}&\includegraphics[width=0.2\linewidth]{fourier_1D/fc-3-mmd/3_30_40/comparison}
\end{tabular}
\caption{$N=30$ and $f_c = 3$. Top row shows the error as we change $\tau$. The results are averaged over $20$ random noisy instances.Bottom row shows the reconstruction for one particular noisy instance. \label{fig:fourier30}}
\end{figure}


\subsection{Microscopy}
Consider
$$
\phi(\Omega,R) = \pa{\exp\pa{-\frac{(\Omega_i-\Omega)^2}{2\sigma^2}} \exp(-R_j R)}_{i\in [M],\; j\in [T]},\qquad (\Omega,R_j)\in [0,1]\times [0,1].
$$




Let the grid size be $N_\Omega = 20$ and $N_R = 5$.
The operator is defined with $\sigma=0.1$, and $M=20$ and $T=3$ uniformly spaced samples on $[0,1]\times [0,1]$. The data is generated from the sparse measure
$$
\mu_0 = 2\delta_{(\Omega+ h_1/M,\; R_1 -h_2/T)} + \delta_{(\Omega-h_1/M,\; R_2 +h_2/T) },
$$
where $ h_1$ and $h_2$ is the fraction that we move inside the grid. The observed signal is
\begin{equation}\label{eq:noisy_y2}
y =  y_0+ \Nn(0, \rho^2 \Id_{MT}), \qwhereq y_0 \eqdef \Phi \mu_0 \qandq \rho \eqdef 0.01 \frac{\norm{y_0}}{\sqrt{MT}}.
\end{equation}
We show the influence of changing $h_1,h_2$ on $(\tau_1,\tau_2)$ and the reconstruction. Given $(h_1,h_2)$, we carry out the following computations:
\begin{enumerate}
\item Find the optimal $\lambda_*$ parameter for Lasso. We do this by searching over a grid of size 10 on $[0,\lambda_{\max}]$ where we let $\lambda_{\max} = \norm{X^\top y_0}_\infty$. For each $\lambda$ value on this grid, we compute
$$
E_{L}(\lambda)\eqdef \frac{1}{5} \sum_{i=1}^{5} D(\mu_0, \mu_{\mathrm{Lasso}}(\lambda,y_i) )
$$
for 10 instances of $y_i$ distribution as in \eqref{eq:noisy_y} and choose  $\lambda_*$ as the parameter with the smallest $E(\lambda)$ value.
\item For this given $\lambda_*$, searching over 100 uniformly spaced points $(\tau_1,\tau_2) \in [0,1]\times [0,1]$, we compute 
$$
E_{SR}(\lambda_*,\tau_1,\tau_2)\eqdef \frac{1}{5} \sum_{i=1}^{5} D(\mu_0, \mu_{\mathrm{SR-Lasso}}(\lambda_*,\tau_1,\tau_2,y_i) )
$$
where the sum is over  5 instances of $y_i$ distribution as in \eqref{eq:noisy_y}. The   $(\tau_{1,*},\tau_{2,*})$   with the smallest $E_{SR}(\lambda_*,\tau_1,\tau_2)$ value is recorded in Table \ref{tab:micros}.
\end{enumerate}
%
We also record in Table \ref{tab:micros} $E_{L}(\lambda_*)$ and $E(\lambda_*,\tau_{1,*},\tau_{2,*})$. One can observe that when $h_1 = 0$ (resp. $h_2 = 0$), the optimal $\tau_1$ (resp. $\tau_2$) parameter is 0, while as we increase $h_1$, $\tau_1$ and also $\tau_2$ are increased to allow for movement inside the grid. The reconstructions are illlustrated in Figures \ref{fig:micros_comp1} and \ref{fig:micros_comp2} where we display the reconstructions for one  instance using the `optimal' $\tau_1$, $\tau_2$ values. Notice from the table that the error for Lasso increases much more as the true spikes move inside grid, whereas the error for SR-Lasso has much milder growth. In figure \ref{fig:micros_tau1} and \ref{fig:micros_tau2}, we plot the  error bars for $\tau_1$ and $\tau_2$. In Figure \ref{fig:micros_tau1}, oberve that when $h_1=0$, the lines as we change $\tau_1$ are all relatively flat, so even thought the optimal $\tau_1$ value is 0 in this, $\tau_1$ has little impact in the reconstruction quality; whereas as we increase $h_1$, $\tau_1$ has a larger impact, with $\tau_1=1$ giving the smallest error. In Figure \ref{fig:micros_tau2}, observe that when $h_2=0$, $\tau_2 = 0$ gives the smallest error, while as soon as $h_2=0.1$, the slope of the lines change and the optimal $\tau_2$ values are close to $\tau_2 =1$.

\setlength{\tabcolsep}{5pt}
\begin{table}
\begin{center}
\begin{tabular}{cc|ccccccc}
$h_1$&$h_2$&$\tau_1^*$&$\tau_2^*$&$\lambda^*$&$E_{\mathrm{L}}(\lambda^*)$&$E_{\mathrm{SR}}(\lambda^*,\tau_1^*,\tau_2^*)$\\
\hline
$0.00$&$0.00$&$0.00$&$0.00$&$0.003421$&$0.00$&$0.001$\\
$0.00$&$0.10$&$0.25$&$0.75$&$0.003421$&$0.18$&$0.053$\\
$0.00$&$0.20$&$1.00$&$0.75$&$0.017633$&$0.33$&$0.043$\\
$0.00$&$0.30$&$0.00$&$1.00$&$0.035958$&$0.45$&$0.054$\\
$0.00$&$0.40$&$0.00$&$1.00$&$0.034211$&$0.53$&$0.056$\\
\hline
$0.10$&$0.00$&$1.00$&$0.00$&$0.010538$&$0.05$&$0.003$\\
$0.10$&$0.10$&$1.00$&$0.75$&$0.010538$&$0.18$&$0.042$\\
$0.10$&$0.20$&$0.50$&$0.75$&$0.018986$&$0.32$&$0.049$\\
$0.10$&$0.30$&$0.50$&$1.00$&$0.034204$&$0.43$&$0.059$\\
$0.10$&$0.40$&$0.50$&$1.00$&$0.034200$&$0.52$&$0.059$\\
\hline
$0.20$&$0.00$&$1.00$&$0.00$&$0.018969$&$0.08$&$0.005$\\
$0.20$&$0.10$&$1.00$&$0.75$&$0.018969$&$0.18$&$0.046$\\
$0.20$&$0.20$&$1.00$&$1.00$&$0.018968$&$0.31$&$0.059$\\
$0.20$&$0.30$&$1.00$&$1.00$&$0.034165$&$0.42$&$0.058$\\
$0.20$&$0.40$&$0.75$&$1.00$&$0.034161$&$0.50$&$0.059$\\
\hline
$0.30$&$0.00$&$1.00$&$0.00$&$0.018938$&$0.11$&$0.024$\\
$0.30$&$0.10$&$1.00$&$0.75$&$0.018938$&$0.18$&$0.061$\\
$0.30$&$0.20$&$1.00$&$1.00$&$0.034101$&$0.30$&$0.062$\\
$0.30$&$0.30$&$1.00$&$1.00$&$0.034098$&$0.41$&$0.062$\\
$0.30$&$0.40$&$1.00$&$1.00$&$0.034093$&$0.49$&$0.062$\\
\hline
$0.40$&$0.00$&$1.00$&$0.00$&$0.018894$&$0.12$&$0.046$\\
$0.40$&$0.10$&$1.00$&$0.50$&$0.018894$&$0.19$&$0.070$\\
$0.40$&$0.20$&$1.00$&$1.00$&$0.034006$&$0.30$&$0.073$\\
$0.40$&$0.30$&$1.00$&$1.00$&$0.034003$&$0.41$&$0.073$\\
$0.40$&$0.40$&$1.00$&$1.00$&$0.033999$&$0.49$&$0.072$
\end{tabular}
\end{center}
\caption{In this table,  for each $h_1, h_2$ pair, we display the $\lambda$ value that gives the smallest Lasso reconstruction error. For this $\lambda$ value, the displayed $\tau_1,\tau_2$ values are the values that give the smallest reconstruction error for SR-Lasso. The corresponding reconstruction errors are displayed for Lasso $E_{\mathrm{L}}$ and SR Lasso $E_{\mathrm{SR}}$. Note that these values are averaged over 10 random noisy observations.
 \label{tab:micros}}
\end{table}


\setlength{\tabcolsep}{0pt}
\begin{figure}
\begin{center}
\begin{tabular}{ccccccc}
&$h_2=0$& $h_2=0.1$&$h_2=0.2$& $h_2=0.3$&$h_2=0.4$\\
\rotatebox{90}{\hspace{15pt}$h_1=0$}&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_0/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_10/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_20/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_30/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_40/tau1_SRLasso}\\
\rotatebox{90}{\hspace{15pt}$h_1=0.1$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_0/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_10/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_20/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_30/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_40/tau1_SRLasso}
\\
\rotatebox{90}{\hspace{15pt}$h_1=0.2$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_0/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_10/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_20/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_30/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_40/tau1_SRLasso}
\\
\rotatebox{90}{\hspace{15pt}$h_1=0.3$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_0/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_10/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_20/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_30/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_40/tau1_SRLasso}
\\
\rotatebox{90}{\hspace{15pt}$h_1=0.4$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_0/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_10/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_20/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_30/tau1_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_40/tau1_SRLasso}
\end{tabular}

\end{center}
\caption{Plot of  $\tau_1$ against reconstruction error. The error bars are the standard deviation over 10 random noisy observations. Each line corresponds to a different $\tau_2$ value.\label{fig:micros_tau1}}

\end{figure}

\begin{figure}
\begin{center}

\begin{tabular}{ccccccc}
&$h_2=0$& $h_2=0.1$&$h_2=0.2$& $h_2=0.3$&$h_2=0.4$\\
\rotatebox{90}{\hspace{15pt}$h_1=0$}&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_0/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_10/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_20/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_30/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_40/tau2_SRLasso}\\
\rotatebox{90}{\hspace{15pt}$h_1=0.1$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_0/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_10/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_20/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_30/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_40/tau2_SRLasso}
\\
\rotatebox{90}{\hspace{15pt}$h_1=0.2$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_0/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_10/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_20/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_30/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_40/tau2_SRLasso}
\\
\rotatebox{90}{\hspace{15pt}$h_1=0.3$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_0/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_10/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_20/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_30/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_40/tau2_SRLasso}
\\
\rotatebox{90}{\hspace{15pt}$h_1=0.4$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_0/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_10/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_20/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_30/tau2_SRLasso}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_40/tau2_SRLasso}
\end{tabular}

\end{center}
\caption{Plot of  $\tau_2$ against reconstruction error. The error bars are the standard deviation over 10 random noisy observations. Each line corresponds to a different $\tau_1$ value.\label{fig:micros_tau2}}


\end{figure}


\begin{figure}
\begin{center}


\begin{tabular}{ccccccc}
&$h_2=0$& $h_2=0.1$&$h_2=0.2$& $h_2=0.3$&$h_2=0.4$\\
\rotatebox{90}{\hspace{15pt}$h_1=0$}&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_0/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_10/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_20/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_30/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_40/comparison_1}\\
\rotatebox{90}{\hspace{15pt}$h_1=0.1$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_0/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_10/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_20/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_30/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_40/comparison_1}
\\
\rotatebox{90}{\hspace{15pt}$h_1=0.2$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_0/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_10/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_20/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_30/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_40/comparison_1}
\\
\rotatebox{90}{\hspace{15pt}$h_1=0.3$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_0/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_10/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_20/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_30/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_40/comparison_1}
\\
\rotatebox{90}{\hspace{15pt}$h_1=0.4$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_0/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_10/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_20/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_30/comparison_1}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_40/comparison_1}
\end{tabular}

\end{center}
\caption{Comparison between Lasso reconstruction and SR-Lasso reconstructions.
\label{fig:micros_comp1}}

\end{figure}


\begin{figure}
\begin{center}

\begin{tabular}{ccccccc}
&$h_2=0$& $h_2=0.1$&$h_2=0.2$& $h_2=0.3$&$h_2=0.4$\\
\rotatebox{90}{\hspace{15pt}$h_1=0$}&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_0/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_10/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_20/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_30/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/0_40/comparison_2}\\
\rotatebox{90}{\hspace{15pt}$h_1=0.1$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_0/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_10/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_20/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_30/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/10_40/comparison_2}
\\
\rotatebox{90}{\hspace{15pt}$h_1=0.2$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_0/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_10/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_20/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_30/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/20_40/comparison_2}
\\
\rotatebox{90}{\hspace{15pt}$h_1=0.3$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_0/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_10/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_20/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_30/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/30_40/comparison_2}
\\
\rotatebox{90}{\hspace{15pt}$h_1=0.4$}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_0/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_10/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_20/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_30/comparison_2}
&\includegraphics[width=0.18\linewidth]{microscopy_mmd/40_40/comparison_2}
\end{tabular}

\end{center}
\caption{Comparison between Lasso reconstruction and SR-Lasso reconstructions.\label{fig:micros_comp2}}
\end{figure}

